Wave-Like Solutions of General One-Dimensional Spatially Coupled Systems

We establish the existence of wave-like solutions to spatially coupled graphical models which, in the large size limit, can be characterized by a one-dimensional real-valued state. This is extended to a proof of the threshold saturation phenomenon for all such models, which includes spatially coupled irregular LDPC codes over the BEC, but also addresses hard-decision decoding for transmission over general channels, the CDMA multiple-access problem, compressed sensing, and some statistical physics models. For traditional uncoupled iterative coding systems with two components and transmission over the BEC, the asymptotic convergence behavior is completely characterized by the EXIT curves of the components. More precisely, the system converges to the desired fixed point, which is the one corresponding to perfect decoding, if and only if the two EXIT functions describing the components do not cross. For spatially coupled systems whose state is one-dimensional a closely related graphical criterion applies. Now the curves are allowed to cross, but not by too much. More precisely, we show that the threshold saturation phenomenon is related to the positivity of the (signed) area enclosed by two EXIT-like functions associated to the component systems, a very intuitive and easy-to-use graphical characterization. In the spirit of EXIT functions and Gaussian approximations, we also show how to apply the technique to higher dimensional and even infinite-dimensional cases. In these scenarios the method is no longer rigorous, but it typically gives accurate predictions. To demonstrate this application, we discuss transmission over general channels using both the belief-propagation as well as the min-sum decoder.

==> reduction.tex <==
\section{Proof for the General Case\label{sec:general}}

In Section \ref{sec:PCcase} we proved Theorem
\ref{thm:PCexist},
a special case of Theorem \ref{thm:mainexist}
in which $\hg$ and $\hf$ are piecewise constant
functions and $\smthker$ is $C_1$ and strictly positive.
In this section we show how to remove the speical conditions 
to arrive at the general results.
We make repeated use of the limit theorems of Section \ref{sec:limitthms} and develop
some approximations for functions in $\exitfns.$
It is quite simple to approximate $h \in \exitfns$ using piecewise constant functions.
The only difficulty is to approximate a pair $(\hg,\hf)$ so that the strictly positive gap
condition is preserved.

\subsection{Approximation by Scaling}
Let $h \in \exitfns$ and denote $\int_0^1 h(x) \, dx$ by $A.$
For $0< a < 1$ we define 
\[
\slanta{h} (x) = h\Bigl(\frac{x - (1-A)}{1-a} + (1-A)\Bigr)
\]
where we assume $h(x)=0$ for $x<0$ and 
$h(x)=1$ for $x>1.$ A quick calculation verifies
$\int_0^1 \slanta{h} (x) dx = A.$
Note that $h(x) \ge \slanta{h}(x)$ for $u \in [0,1-A]$ and 
that $h(x) \le \slanta{h}(x)$ for $x \in [1-A,1].$
It follows that 
$0 \le \int_0^z (h(x)-\slanta{h}(x))\, dx \le \frac{a}{1-a}\int_0^{1-A} h(x)\,dx$
for all $z \in [0,1],$
which yields
$\Phi(\hg,\hf) \le \Phi(\slanta{\hg},\slanta{\hf})$ and
$E(\hg,\hf) = E(\slanta{\hg},\slanta{\hf}).$

\begin{lemma}\label{lem:smoothcompress}
Let $(\hg,\hf) \in \exitfns^2$ 
satisfy the strictly positive gap condition.
Then, there exists $\epsilon > 0$ such that
$(\slanta{\hg},\slanta{\hf})$ 
satisfies the strictly positive gap condition
for any $a \in (0,\epsilon).$
\end{lemma}
\begin{IEEEproof}[Proof of Lemma \ref{lem:smoothcompress}]
Let $A_1 = \int_0^1 \hg(x) dx,$ $A_2 = \int_0^1 \hf(x) dx$ so $E(\hg,\hf) = 1-A_1-A_2.$
By symmetry we need only consider the case $E \ge 0.$

First, we note that 
$[0,a (1-A_1)]\times [0,a (1-A_2)]\subset \gapptsplus(\slanta{\hg},\slanta{\hf})$ 
and
$[1-a A_1,1]\times [1-a A_2,1]\subset \gapptsminus(\slanta{\hg},\slanta{\hf}).$
Thus, it remains only to show that $\Phi(\slanta{\hg},\slanta{\hf}) > E$ on 
$\intcross(\slanta{\hg},\slanta{\hf}).$
Assume $v \in \intcross(\slanta{\hg},\slanta{\hf}).$ 
%Our aim is to show that $\Phi(\slanta{\hg},\slanta{\hf};v_1,v_2) > E.$

Let $\eta$ be chosen with $0 < \eta < \min\{A_1,A_2,1-A_1,1-A_2\}.$
Define
\[
\tilde{\cross}(\hg,\hf) = \cross(\hg,\hf) \backslash (\ball_{\eta/2}(0,0) \cup \ball_{\eta/2}(1,1)).
\]
By continuity, there exists $\gamma >0,$ which we may take to be less than $2\eta,$
such that
$\Phi(\hg,\hf) > \gamma + E$ on $\tilde{\cross}(\hg,\hf).$
Since $\Phi$ is Lipschitz-1 in its last two arguments it follows that
$\Phi(\hg,\hf) > \gamma/2 + E$ on $\neigh{\tilde{\cross}(\hg,\hf)}{\gamma/4}.$
For all $a$ sufficiently small we have
$|\Phi(\hg,\hf) - \Phi(\slanta{\hg},\slanta{\hf})| < \gamma/2$ uniformly
and it follows that  
$\Phi(\slanta{\hg},\slanta{\hf}) > E$ on $\neigh{\tilde{\cross}(\hg,\hf)}{\gamma/4}.$
By Lemma \ref{lem:crosspointlimit}, for all $a$ sufficiently small we have
\(
{\cross}(\slanta{\hg},\slanta{\hf})
\subset \neigh{{\cross}(\hg,\hf)}{\gamma/4}
\)
and since
\(
\neigh{{\cross}(\hg,\hf)}{\gamma/4}
\subset
\ball_{\eta}(0,0) \cup \ball_{\eta}(1,1) \cup \neigh{\tilde{\cross}(\hg,\hf)}{\gamma/4}
\)
we have
\[
{\cross}(\slanta{\hg},\slanta{\hf})
\subset 
\ball_{\eta}(0,0) \cup \ball_{\eta}(1,1) \cup \neigh{\tilde{\cross}(\hg,\hf)}{\gamma/4}\,.
\]
Therefore, it remains only to bound 
$\Phi(\slanta{\hg},\slanta{\hf}; v)$ on $\ball_{\eta}(0,0) \cup \ball_{\eta}(1,1).$

Since $\Phi(\hg,\hf) \le \Phi(\slanta{\hg},\slanta{\hf})$ it is sufficient to show
$\Phi(h_{1},h_{2};v_1,v_2) > E,$ or equivalently
$\hat{\Phi}(h_{1},h_{2};v_1,v_2) > 0.$
If $v\in \cross(\hg,\hf)$ then the inequality is immediate, so we assume
$v\not\in \cross(\hg,\hf).$
If $(v_1,v_2) \le (1-A_1,1-A_2)$ 
then since $v_1 \in \closure{h}_{2,a}(v_2)$ we have
$v_1 \le \hf(v_2^+)$ and, similarly, $v_2 \le \hg(v_1^+),$ hence
$v \in \gapptsminus(\hg,\hf).$
Similarly, if $(v_1,v_2) \ge (1-A_1,1-A_2)$ 
then $v \in \gapptsplus(\hg,\hf).$

Since $\closeM[\hg,\hf](v) \in \cross(\hg,\hf)$ and 
$v\not\in \cross(\hg,\hf),$ 
Lemma \ref{lem:verphigap} and Lemma \ref{lem:Rvverify}
%Lemma \ref{lem:Mphigap} 
yield
${\Phi}(\hg,\hf;\closeM(v)) > {\Phi}(\hg,\hf;v)$
and, equivalently,
$\hat{\Phi}(\hg,\hf;\closeM(v)) < \hat{\Phi}(\hg,\hf;v).$

Assume $v\in \ball_\eta(0,0).$ 
Then $v \in \gapptsminus(\hg,\hf)$ and $\closeM(v) \le v.$
We cannot have $\closeM(v)=(0,0)$ since ${\Phi}(\hg,\hf;0,0)=0$ and
${\Phi}(\hg,\hf;v) > 0$ (by Lemma \ref{lem:PhiEquiv}).
Hence $\closeM[\hg,\hf](v) \in \intcross(\hg,\hf),$ 
which implies $\hat{\Phi}(\hg,\hf;\closeM(v)) > 0,$ and we obtain
$\hat{\Phi}(\hg,\hf;v) > 0.$

Now consider the case $v\in \ball_\eta(1,1).$ 
Then $v \in \gapptsplus(\hg,\hf)$ and $\closeM(v) \ge v.$
It follows directly that $\hat{\Phi}(\hg,\hf;\closeM(v)) \ge 0$ (although we could show
that $\closeM(v) \neq (1,1)$ and that the inequality is strict)
and we obtain $\hat{\Phi}(\hg,\hf;v) > 0.$
\end{IEEEproof}

\subsection{Piecewise Constant Approximation}
Given any $h \in \exitfns$ let us define a sequence of piecewise constant approximations
$Q_n(h),$ $n=1,2,...$  by
\(
Q_n(h) (x) = \sum_{j=1}^n \frac{1}{n} \,1_{x \ge u_{n,j}}
\)
where we set 
\[
u_{n,j} =  \int_0^1 \max\{ (n h(x) - (j-1))^+,1 \} dx.
\]
If $h$ is invertible then we have $u_{n,j} = n\int_{(j-1)/n}^{j/n}(1-h^{-1}(x))dx$
and 
\(
\int_0^1 Q_n(h) (x) dx = \sum_{j=1}^n \frac{1-u_{n,j}}{n} = \int_0^1 (1-h^{-1})(x) dx = \int_0^1 h (x) dx.
\)
In general, it holds that
\(
\int_0^1 Q_n(h) (x) dx = \int_0^1 h (x) dx.
\)
Since $h$ is non-decreasing, it also follows that $\int_0^z Q_n(h) (x) dx \le \int_0^z h (x) dx$ for all
$z \in [0,1].$
%\begin{IEEEproof}
%In general, let $(x_j,\frac{j}{i}) \in \closure{h}$ where we may assume $x_i =1.$
%Then $x_j \ge u_{i,j}$ and $\int_0^{x_j} h_i(x) dx = \int_0^{x_j} h(x) dx.$
%Furthermore, it is an easy exercise to show that,
%among all non-decreasing functions satisfying these integral equality conditions,
%$h_i$ minimizes $\int_0^z h_i(x) dx$ for all $z.$
%\end{IEEEproof}

\begin{lemma}\label{lem:PCapprox}
Let $(\hg,\hf)$ be pair of functions in $\exitfns$ satisfying the strictly positive gap condition 
such that for some $\eta>0$ we have
$\hg (x) =\hf(x)= 0$ for
$x \in [0,\eta)$ and $\hg (x) =\hf(x)= 1$ for $x \in (1-\eta,1].$
Then, for all $n$ sufficiently large $n,$
$(Q_n(\hg),Q_n(\hf))$ satisfies the strictly positive gap condition.
\end{lemma}
\begin{IEEEproof}
By symmetry we need only consider the case $E(\hg,\hf) \ge 0.$

Since $\hg$ and $\hf$ are $0$ on $[0,\eta)$ and $(1-\eta,1]$ it follows that 
$\intcrossing (\hg,\hf) \subset [\eta,1-\eta]^2.$
Further, $\intcrossing (\hg,\hf)$ is closed and there exists $\gamma > 0$ such that 
$\Phi(\hg,\hf;v_1,v_2) \ge \gamma + E$ on $\intcrossing (\hg,\hf).$
Since $\Phi(\hg,\hf)$ is Lipschitz-1 componentwise it follows that 
$\Phi(\hg,\hf) > \gamma/2 + E$ on $\neigh{\intcrossing (\hg,\hf)}{\gamma/4}.$
Observe that $\Phi(Q_n(h_{1}),Q_n(h_{2}))$ converges in $n$ uniformly to $\Phi(\hg,\hf).$
(In fact we have $0 \le |\Phi(\hg,\hf)-\Phi(Q_n(h_{1}),Q_n(h_{2}))| \le \frac{1}{n}.$)
So, for $n$ sufficiently large, we have $\Phi(Q_n(h_{1}),Q_n(h_{2})) > E$ on 
$\neigh{\intcrossing (\hg,\hf)}{\gamma/4}.$
By construction we also have $\intcrossing (Q_n(h_{1},Q_n(h_{2})) \in [\eta,1-\eta]^2.$
By Lemma \ref{lem:crosspointlimit} we now have 
\(
\intcrossing (Q_n(h_{1}),Q_n(h_{2})) \subset 
\neigh{\intcrossing (h_{1},h_{2})}{\gamma/4}
\)
for all $n$ sufficiently large so $\Phi(Q_n(h_{1}),Q_n(h_{2})) > E$ on
$\intcrossing (Q_n(h_{1}),Q_n(h_{2})).$

Finally, we note that $[0,\eta]^2 \subset \gapptsplus(Q_n(h_{1}),Q_n(h_{2}))$
and $[1-\eta,1]^2 \subset \gapptsminus(Q_n(h_{1}),Q_n(h_{2})).$
This completes the proof.
\end{IEEEproof}

\subsection{Proof of Main Results}

We are now ready to prove our main results.

\begin{IEEEproof}[Proof Theorem \ref{thm:mainexist}]
The proof proceeds by repeated application of Lemma \ref{lem:limitexist}
to establish existence of $f,g \in \Psi$ and constant $\ashift$ such that
$h^{\fS,g} = \hg$ and $h^{\gSa,f} = \hf$ for a series of 
increasingly generalized cases of $(\hg,\hf)$ and $\smthker.$
The simplest case is already establishted in Thereom \ref{thm:PCexist}.

We first generalize to arbitrary $\smthker.$
Assume that $(\hg,\hf)$ are both piecewise constant.
Define $\smthker_i = \smthker \otimes G_i$ where 
$G_i(x) = \frac{i}{\sqrt{2\pi}} e^{- (ix)^2/2}.$
It follows that $\smthker_i \rightarrow \smthker$ in $L_1$
and $\| \smthker_i \|_\infty \le \| \smthker\|_\infty.$
For each $\smthker_i$ we apply Theorem \ref{thm:PCexist}
to obtain piecewise constant $f_i,g_i \in \Psi$ 
(with corresponding $\zfi,\zgi$) and constants $\ashift_i$
such that $h^{f_i^{{\smthker}_i},g_i} = \hg$ and $h^{g_i^{{\smthker}_i,\ashift_i},f_i} = \hf.$
We can now apply Lemma \ref{lem:limitexist} as indicated above to conclude
existence for general $\smthker.$

We now generalize $(\hg,\hf)$ and to
require, beyond the conditions of the Theorem statement, only that there exists $\eta > 0$ such that $\hg (x) =\hf(x)= 0$ for
$x \in [0,\eta)$ and $\hg (x) =\hf(x)= 1$ for $x \in (1-\eta,1].$
We apply Lemma \ref{lem:PCapprox} and the preceding case already established
to conclude that for all $n$ sufficiently large
there exists (piecewise constant) $f_n,g_n \in \Psi$ and finite constants $\ashift_n$ such that
$h^{f_n^{{\smthker}},g_n} = Q_n(\hg)$ and $h^{g_n^{{\smthker},\ashift_n},f_n} = Q_n(\hf).$
Since $Q_n(\hg)$ and $Q_n(\hf)$ converge to $\hg$ and $\hf$ respectively,
we can apply Lemma \ref{lem:limitexist} to conclude existence for this case.

For arbitrary $(\hg,\hf)$ we consider $(\slanta{\hg},\slanta{\hf}).$
We apply Lemma \ref{lem:smoothcompress} and the preceding case to conclude that for all $a$ sufficiently small
there exists $f_a,g_a \in \Psi$ and finite constants $\ashift_a$ such that
$h^{f_a^{{\smthker}},g_a} = \slanta{\hg}$ and $h^{g_a^{{\smthker},\ashift_a},f_a} = \slanta{\hf}.$
We make a final application of Lemma \ref{lem:limitexist} to obtain a solution for the general case.

In all cases above the approximations used preserve $E.$
In particular, if $E(\hg,\hf) = 0$ then we have respectively,
$\ashift_i=0$ or $\ashift_n=0$ of $\ashift_a=0$ and we obtain $\ashift=0$
from the limit construction in Lemma \ref{lem:limitexist}.
If $E(\hg,\hf) \neq 0$ then we cannot have $\ashift=0$ by Lemma \ref{lem:PPhi}.
Moreover, we must have $\sgn (E) = \sgn (\ashift).$
Finally, the bound $|\ashift| \ge |E|/\|\smthker\|_\infty$ was proved in Lemma \ref{lem:shiftbound}.
\end{IEEEproof}


